MLC for parabolically bounded primitive renormalization

We prove $\textit{a priori}$ bounds and MLC (local connectivity of the Mandelbrot set $\mathcal{M}$) for a class of infinitely renormalizable parameters whose renormalization type is primitive but can approach the cusp of $\mathcal{M}$. To this end we develop and refine a variety of tools that allow us to control degeneration of renormalizations. They include the Thin-Thick Decomposition, the Value Calculus, the Wanderers Theorem, and the Wave Lemma.

==> macros/basic_style_macros.tex <==
\input{macros/packages}
\input{macros/theorem_types}


==> macros/group_macros.tex <==
%% Macros for some Lie groups and homogenous spaces, along with a bit of related notation. 
\DeclareMathOperator{\PGL}{PGL}
\DeclareMathOperator{\PSO}{PSO}
\DeclareMathOperator{\PSL}{PSL}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\Fix}{Fix}


\renewcommand{\H}{\mathbb H}


==> macros/long_submission_macros.tex <==
% These are the macros for a long submission with sections and hard page limits
\numberwithin{equation}{section}
\input{macros/packages}
\input{macros/theorem_types}
\input{macros/formula_macros}


==> macros/note_macros.tex <==
% These are the macros for a note with no sections and no hard page limits
\usepackage[margin=1.5in]{geometry}
\input{macros/packages}
\input{macros/theorem_types}
\input{macros/formula_macros}


==> macros/short_submission_macros.tex <==
% This gives you the macros for a short submission with no sections and hard page limits
% You should set the geometry yourself to fit the page limits
\input{macros/basic_style_macros}
\input{macros/formula_macros}

==> macros/simons_style_macros.tex <==
% This file is now deprecated in favor of basic_style_macros.tex
% It can be used for submissions with no sections and hard page limits
\input{macros/basic_style_macros}

==> macros/style_macros.tex <==
% This file is now deprecated and exists only for backward compatibility
% It was meant to be used for a longer paper with sections and no hard page limits
\input{macros/paper_style_macros}
\input{macros/basic_style_macros}


==> misha-macros.tex <==
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem{obs}[thm]{Observation}
%\theoremstyle{remark}
%\newtheorem{rem}{Remark}[section]
%\newtheorem{notation}{Notation}
%\newtheorem{exc}[thm]{Exercise}
%\newtheorem{exe}[thm]{Exercise}
%\newtheorem{problem}[thm]{Problem}

%\theoremstyle{definition}
%\newtheorem{defn}{Definition}[section]

%\theoremstyle{plain}
%\newtheorem*{thmA}{Main Theorem (physical version)}
%\newtheorem*{thmB}{Main Theorem (dynamical version)}
%\newtheorem*{thmC}{Theorem (Global Lee-Yang-Fisher Current)}
%\newtheorem*{thmRIG}{Local Rigidity Theorem}
%\newtheorem*{LY Theorem}{Lee-Yang Theorem}
%\newtheorem*{LY Theorem2}{General Lee-Yang Theorem}
%\newtheorem*{LY TheoremBC}{Lee-Yang Theorem with Boundary Conditions}
%\newtheorem*{LY Theorem2BC}{General Lee-Yang Theorem with Boundary Conditions}
%\newtheorem*{conj}{Conjecture}

\numberwithin{equation}{section}
\numberwithin{figure}{section}

\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\Rmig}{R} %the Migdal-Kadinoff renormalization in U,V,W coords.
\newcommand{\Cmig}{C} %the invariant ``cylinder'' for \Rmig
\newcommand{\Cmigbl}{C_0}
\newcommand{\TOPmig}{\mathrm{T}} %the invariant ``cylinder'' for \Rmig
\newcommand{\BOTTOMmig}{\mathrm{B}} %the invariant ``cylinder'' for \Rmig
%fixed points:
\newcommand{\FIXmig}{b} %the fixed points on the invariant ``cylinder'' for \Rmig
\newcommand{\CFIXmig}{e} %the complex attacting fixed points for \Rmig
%indeterminant points:
\newcommand{\INDmig}{a} %the indeterminant points for \Rmig
\newcommand{\Smig}{S} %the principal locus for \Rmig, i.e. the line U+2V+W=0

\newcommand{\thin} {{\mathrm{thin}}}
\newcommand{\thick} {{ \mathrm{thick}}}
\newcommand{\loc}{{\mathrm {loc}}}
\newcommand{\hor}{{\mathrm {hor}}}
\newcommand{\ver}{{\mathrm {ver}}}
\newcommand{\ess}{{\mathrm{ess}}}
\newcommand{\ness}{{\mathrm{ne}}}
\newcommand{\pro}{{\mathrm{pr}}}

\newcommand{\locflux} {\WW^\perp_\loc}

\newcommand{\re}{{\mathrm{(r)}}}
\newcommand{\essre}{{\mathrm{ess(r)}}}
\newcommand{\nere}{{\mathrm{ne(r)}}}
\newcommand{\verre}{{\mathrm{ver(r)}}}

\newcommand{\Cyl}{{\mathrm{Cyl}}}
\newcommand{\hsubset}{{ \,\underset{h}{\subset}\, }    }
\newcommand{\hsupset}{{ \, \underset{h}{\supset} \, }     }

% \newcommand{\lp}{\multimap}
\newcommand{\lp}{{\,\mathrm {dominates}\,}}



\newcommand{\Rphys}{\mathcal R} %the Physical renormalization in Z,T,S coords.
\newcommand{\Cphys}{\mathcal C} %the invariant cylinder for \Rphys
\newcommand{\Solid}{\mathcal{SC}}
\newcommand{\Solidmig}{SC}
\newcommand{\Secphys}{\Pi}
\newcommand{\Secmig}{P}
\newcommand{\TOPphys}{\mathcal T} %Top the invariant cylinder for \Rphys
\newcommand{\Cphystl}{{\mathcal C}_1}
\newcommand{\Cphysbl}{{\mathcal C}_0}
\newcommand{\Cphyslow}{{\mathcal C}_*}
\newcommand{\BOTTOMphys}{\mathcal B} %Top the invariant cylinder for \Rphys
%fixed points:
\newcommand{\FIXphys}{\beta} %the fixed points on the invariant cylinder for \Rphys
\newcommand{\CFIXphys}{\eta} %the complex attacting fixed points for \Rphys
%indeterminant points:
\newcommand{\INDphys}{\alpha} %the indeterminant points for \Rmig
\newcommand{\Sphys}{\mathcal S} %the principal locus for \Rphys, i.e. the curve line z^2+2zt+1=0
\newcommand{\Icurve}{\mathcal G} %image of the indeterminacy pts
\newcommand{\Imig}{G} 
\newcommand{\PI}{{\mathcal A}}
\newcommand{\crittemps}{{\mathscr C}} %The set of all critical tempuratures
\newcommand{\epoints}{{\mathscr E}} %The set of all endpoints of high-tempurature hairs


\newcommand{\Line}{L}
\newcommand{\Lzero}{L_0}
\newcommand{\Lone}{L_1}
\newcommand{\Ltwo}{L_2}
\newcommand{\Lthree}{L_3}
\newcommand{\Lfour}{L_4}

\newcommand{\LLzero}{\LL_0}
\newcommand{\LLone}{\LL_1}

\newcommand{\Div}{{\rm Div}}
\newcommand{\Tongue}{\Upsilon}

\newcommand{\Par}{{{\mathcal P}}}
\newcommand{\inv}{{\iota}}

\newcommand{\leg}{{\mathrm {leg}}}
\newcommand{\il}{{\mathrm {il}}}

\newcommand{\Mconv}{{\rm M}}
\newcommand{\Hconv}{{\rm H}}
\newcommand{\tconv}{{\rm t}}

\newcommand{\Weight}{W}

\newcommand{\KSQRT}{\widehat \KK}

\newcommand{\ex}{{\mathrm{exc}}}
\newcommand{\out}{{\mathrm{out}}}

\newcommand{\vertbondpp}{\, \underset{\oplus}{\overset{\oplus}{|}} \, }
\newcommand{\vertbondpm}{\, \underset{\ominus}{\overset{\oplus}{|}} \,}
\newcommand{\vertbondmp}{\, \underset{\oplus}{\overset{\ominus}{|}} \, }
\newcommand{\vertbondmm}{\, \underset{\ominus}{\overset{\ominus}{|}} \, }

%\newcommand{\vertpp}{\, \underset{\oplus}{\overset{\oplus}{ \Diamond} } \, }
%\newcommand{\vertpm}{\, \underset{\ominus}{\overset{\oplus}{\Diamond}} \, }
%\newcommand{\vertmp}{\, \underset{\oplus}{\overset{\ominus}{\Diamond}} \, }
%\newcommand{\vertmm}{\, \underset{\ominus}{\overset{\ominus}{\Diamond}}\,}

\font\nt=cmr7

%\def\note#1
%{\marginpar
%{\nt $\leftarrow$
%\par
%\hfuzz=20pt \hbadness=9000 \hyphenpenalty=-100 \exhyphenpenalty=-100
%\pretolerance=-1 \tolerance=9999 \doublehyphendemerits=-100000
%\finalhyphendemerits=-100000 \baselineskip=6pt
%#1}\hfuzz=1pt}

\def\note#1{}

% \newcommand{\bignote}[1]{\begin{quote} \sf #1 \end{quote}}

\long\def\bignote#1{}


% \centerline{NEW MACROS (2019) } 

\newcommand{\lo}{{\mathrm{lo}}}
\newcommand{\lobr}{{\mathrm{lo-br}}}
\newcommand{\sh}{{\mathrm{sh}}}
\newcommand{\sei}{{\mathrm{si}}}
\newcommand{\pe}{{\mathrm{pe}}}

\newcommand{\ol}{\overline}
\newcommand{\ul}{\underline}

% \newcommand{\pp}{{\partial}}
\newcommand{\pp}{{\mathfrak{p}}}
\newcommand{\qq}{{\mathfrak{q}}}
\newcommand{\bb}{{\mathfrak{b}}}



\newcommand{\Kfilled}{{\mathcal {K} }}
\newcommand{\Jul}{{\mathcal{J}}}
\newcommand{\Sec} {{{S}}}
\newcommand{\Zec} {{{Z}}}
% \newcommand{\Zay}{{\mathcal{?}}}
\newcommand{\Hub}{\TT}

% \centerline{OLD MACROS continued} 




%Commands specific to the renormalization operators:



\newcommand{\QED}{\rlap{$\sqcup$}$\sqcap$\smallskip}

\def\sss{\subsubsection}

\newcommand{\correspond}{\Psi}
\newcommand{\conjugacy}{\psi}

\newcommand{\rank}{\rm rank}
\newcommand{\di}{\partial}
\newcommand{\dibar}{\bar\partial}
\newcommand{\hookra}{\hookrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\hra}{\hookrightarrow}
\newcommand{\imply}{\Rightarrow}
\def\lra{\longrightarrow}
\newcommand{\wc}{\underset{w}{\to}}
\newcommand{\tu}{\textup}

%\newcommand{\hor}{{ah}}
%\newcommand{\ver}{{av}}



\def\ssk{\smallskip}
\def\msk{\medskip}
\def\bsk{\bigskip}
\def\noi{\noindent}
\def\nin{\noindent}
\def\lqq{\lq\lq}
\def\sm{\setminus}
% \def\sm{\smallsetminus}
\def\bolshe{\succ}
\def\ssm{\smallsetminus}
\def\tr{{\text{tr}}}
\def\Crit{{\mathrm{Crit}}}

\newcommand{\ctg}{\operatorname{ctg}}
%\renewcommand{\thenotation}{} 
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\Hdist}{\operatorname{H-dist}}
%\newcommand{\det}{\operatorname{det}}
\newcommand{\cl}{\operatorname{cl}}
\newcommand{\inter}{\operatorname{int}}
\renewcommand{\mod}{\operatorname{mod}}
\newcommand{\card}{\operatorname{card}}
\newcommand{\tl}{\tilde}
\newcommand{\ind}{ \operatorname{ind} }
\newcommand{\Dist}{\operatorname{Dist}}
\newcommand{\Graph}{\operatorname{Graph}}
\newcommand{\len}{\operatorname{\l}}
\newcommand{\vol}{\operatorname{vol}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

%\newcommand{\arg}{\operatorname{arg}}
\newcommand{\orb}{\operatorname{orb}}
\newcommand{\HD}{\operatorname{HD}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\length}{\operatorname{length}}
\newcommand{\dens}{\operatorname{dens}}
\newcommand{\meas}{\operatorname{meas}}
\newcommand{\area}{\operatorname{area}}
\newcommand{\per}{\operatorname{per}}
\renewcommand{\Im}{\operatorname{Im}}

\renewcommand{\d}{{\diamond}}

\newcommand{\lef}{{\mathrm{left}}}
\newcommand{\righ}{{\mathrm{right}}}

\newcommand{\Dil}{\operatorname{Dil}}
\newcommand{\Ker}{\operatorname{Ker}}
\newcommand{\tg}{\operatorname{tg}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\isom}{\approx}
\newcommand{\comp}{\circ}
\newcommand{\esssup}{\operatorname{ess-sup}}
\newcommand{\Rat}{{\mathrm{Rat}}}
\newcommand{\hot}{{\mathrm{h.o.t.}}}
\newcommand{\Conf}{{\mathrm{Conf}}}
% \newcommand{\Top}{{\mathrm{T}}}
%\newcommand{\Bottom}{{\mathrm{B}}}

\newcommand{\SLa}{\underset{\La}{\Subset}}

\newcommand{\const}{\mathrm{const}}
\def\loc{{\mathrm{loc}}}
\def\fib{{\mathrm{fib}}}
\def \br{{\mathrm{br}}}

\newcommand{\eps}{{\epsilon}}
\newcommand{\epsi}{{\epsilon}}
\newcommand{\veps}{{\varepsilon}}

\newcommand{\Ga}{{\Gamma}}
\newcommand{\De}{{\Delta}}
\newcommand{\de}{{\delta}}
\newcommand{\la}{{\lambda}}
\newcommand{\La}{{\Lambda}}
\newcommand{\si}{{\sigma}}
\newcommand{\Si}{{\Sigma}}
\newcommand{\Om}{{\Omega}}
\newcommand{\om}{{\omega}}
\newcommand{\Ups}{{\Upsilon}}

\newcommand{\al}{{\alpha}}
\newcommand{\ba}{{\mbox{\boldmath$\alpha$} }}
\newcommand{\be}{{\beta}}
\newcommand{\bbe}{{\mbox{\boldmath$\beta$} }}
\newcommand{\bk}{{\boldsymbol{\kappa}}}
\newcommand{\bg}{{\boldsymbol{\gamma}}}

\newcommand{\bare}{{\bar\eps}}

\newcommand{\Ray}{{\mathcal R}}
\newcommand{\Eq}{{\mathcal E}}
\newcommand{\PR}{PR}

\newcommand{\AAA}{{\mathcal A}}
\newcommand{\BB}{{\mathcal B}}
\newcommand{\CC}{{\mathcal C}}
\newcommand{\DD}{{\mathcal D}}
\newcommand{\EE}{{\mathcal E}}
\newcommand{\EEE}{{\mathcal O}}
\newcommand{\II}{{\mathcal I}}
\newcommand{\FF}{{\mathcal F}}
\newcommand{\GG}{{\mathcal G}}
\newcommand{\JJ}{{\mathcal J}}
\newcommand{\HH}{{\mathcal H}}
\newcommand{\KK}{{\mathcal K}}
\newcommand{\LL}{{\mathcal L}}
\newcommand{\MM}{{\mathcal M}}
\newcommand{\NN}{{\mathcal N}}
\newcommand{\OO}{{\mathcal O}}
\newcommand{\PP}{{\mathcal P}}
\newcommand{\QQ}{{\mathcal Q}}
\newcommand{\QM}{{\mathcal QM}}
\newcommand{\QP}{{\mathcal QP}}
\newcommand{\QL}{{\mathcal Q}}

\newcommand{\RR}{{\mathcal R}}
\newcommand{\SSS}{{\mathcal S}}
\newcommand{\TT}{{\mathcal T}}
\newcommand{\TTT}{{\mathcal P}}
\newcommand{\UU}{{\mathcal U}}
\newcommand{\VV}{{\mathcal V}}
\newcommand{\WW}{{\mathcal W}}
\newcommand{\XX}{{\mathcal X}}
\newcommand{\YY}{{\mathcal Y}}
\newcommand{\ZZ}{{\mathcal Z}}

\newcommand{\AS}{{\mathcal{AS}}}
\newcommand{\SAS}{{\mathcal{SAS}}}

\newcommand{\A}{{\Bbb A}}
\newcommand{\BBB}{{\Bbb B}}
\newcommand{\C}{{\Bbb C}}
\newcommand{\bC}{{\bar{\Bbb C}}}
\newcommand{\D}{{\Bbb D}}
\newcommand{\Hyp}{{\Bbb H}}
\newcommand{\J}{{\Bbb J}}
\newcommand{\Ll}{{\Bbb L}}
\renewcommand{\L}{{\Bbb L}}
\newcommand{\M}{{\Bbb M}}
\newcommand{\N}{{\Bbb N}}
\newcommand{\Q}{{\Bbb Q}}
\newcommand{\R}{{\Bbb R}}
\newcommand{\T}{{\Bbb T}}
\newcommand{\V}{{\Bbb V}}
\newcommand{\U}{{\Bbb U}}
\newcommand{\W}{{\Bbb W}}
\newcommand{\X}{{\Bbb X}}
\newcommand{\Z}{{\Bbb Z}}



\newcommand{\tT}{{\mathrm{T}}}
\newcommand{\tD}{{D}}
\newcommand{\hyp}{{\mathrm{hyp}}}
\newcommand{\cusp}{{\mathrm{cusp}}}

\newcommand{\fix}{{b}}
\newcommand{\cxfix}{{\xi}}
\newcommand{\LINV}{L_{\rm inv}}
\newcommand{\LLINV}{{\mathcal L}_{\rm inv}}
\newcommand{\f}{{\bf f}}
\newcommand{\g}{{\bf g}}
\newcommand{\h}{{\bf h}}
\renewcommand{\i}{{\bar i}}
\renewcommand{\j}{{\bar j}}

\newcommand{\geoD}{{\boldsymbol{\gamma}}}


%\newcommand{\k}{\kappa}



\newcommand{\Bf}{{\mathbf{f}}}
\newcommand{\Bg}{{\mathbf{g}}}
\newcommand{\Bh}{{\mathbf{h}}}
\newcommand{\Bi}{{\mathbf{i}}}
\def\BJ{{\mathbf{J}}}
\def\Bl{{\mathbf{l}}}
\def\Bm{{\mathbf{m}}}
\def\Bn{{\mathbf{n}}}


\def\Bj{{\mathbf{j}}}
\def\BJ{{\mathbf{J}}}
\def\Bphi{{\mathbf{\Phi}}}
\def\Bpsi{{\mathbf{\Psi}}}
\newcommand\Bom{\boldsymbol{\om}}



\newcommand{\BD}{{\boldsymbol{D}}}
\newcommand{\BE}{{\boldsymbol{E}}}
\newcommand{\BF}{{\boldsymbol{F}}}
\newcommand{\BG}{{\mathbf{G}}}
\def\BH{{\mathbf{H}}}
\newcommand{\BI}{{\boldsymbol{I}}}
\newcommand{\BK}{\mathbf{K}}
\newcommand{\BL}{\mathbf{L}}
\def\B0{{\mathbf{0}}}
\newcommand{\BP}{{\boldsymbol{P}}}
\newcommand{\BS}{{\boldsymbol{S}}}
\def\BT{{\mathbf{T}}}
\newcommand{\BW}{{\mathbf{W}}}
\newcommand{\BV}{{\mathbf{V}}}
\newcommand{\BOM}{{\boldsymbol{\Om}}}



\newcommand{\BPi}{{\boldsymbol{\Pi}}}
\def\BUps{{\boldsymbol{\Upsilon}}}
\def\BLa{{\boldsymbol{\La}}}
\def\BGa{{\boldsymbol\Gamma}}
\def\BDe{{\boldsymbol\Delta}}
\def\BUps{{\boldsymbol\Upsilon}}
\def\BThe{{\boldsymbol\Theta}}
\def\BOm{{\boldsymbol \Om}}
\def\BPsi{{\boldsymbol\Psi}}

\def\Baleph{{\boldsymbol\aleph}}

\newcommand{\Bw}{{\mathbf{w}}}
\newcommand{\Bal}{{\boldsymbol{\alpha}}}
\newcommand{\Bde}{{\boldsymbol{\delta}}}
\newcommand{\Bga}{{\boldsymbol{\gamma}}}
\newcommand{\Bsi}{{\boldsymbol{\sigma}}}
\newcommand{\Bla}{{\boldsymbol{\lambda}}}
\def\Be{\mathbf{e}}
\def\Dia{{\Diamond}}

\def\SB{{\boldsymbol{\BB}}}

\def\ext{{\mathrm{ex}}}
\def\mouth{\operatorname{mouth}}
\def\tail{\operatorname{tail}}

\newcommand{\Comb}{{\it Comb}}
\newcommand{\Top}{{\operatorname{Top}}}
\newcommand{\Bottom}{{\operatorname{Bot}}}
\newcommand{\QC}{\mathcal QC}
\newcommand{\Def}{\mathcal Def}
\newcommand{\Teich}{\mathcal Teich}
%\newcommand{\QL}{{\mathcal{QG}}}
\newcommand{\PPL}{{\mathcal P}{\mathcal L}}
\newcommand{\Jac}{\operatorname{Jac}}
%\newcommand{\DH}{\operatorname{DH}}
\newcommand{\Homeo}{\operatorname{Homeo}}
\newcommand{\AC}{\operatorname{AC}}
\newcommand{\Dom}{\operatorname{Dom}}
\newcommand{\ord}{\operatorname{ord}}


\newcommand{\Hol}{{\rm Hol}}

\newcommand{\Aff}{\operatorname{Aff}}
\newcommand{\Euc}{\operatorname{Euc}}
\newcommand{\MobC}{\operatorname{M\ddot{o}b}({\Bbb C}) }
\newcommand{\PSL}{ {\mathcal{PSL}} }
\newcommand{\SL}{ {\mathcal{SL}} }
\newcommand{\CP}{ {\Bbb{CP}}   }


\newcommand{\hf}{{\hat f}}
\newcommand{\hz}{{\hat z}}
\newcommand{\hM}{{\hat M}} 


\renewcommand{\lq}{``}
\renewcommand{\rq}{''}

\newcommand{\Ch}{\textrm{Ch}}
% \newcommand{\Ch}{{\textrm{\cyr CH} }}


%&&&&&&&&&&    Content   &&&&&&&&


\catcode`\@=12

\def\Empty{}
\newcommand\oplabel[1]{
  \def\OpArg{#1} \ifx \OpArg\Empty {} \else
  	\label{#1}
  \fi}
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Insert a postscript figure using psfig.
% Usage:	\realfig{label}{filename}{caption}
%
% uses psfig macros: must have \input{psfig} in the preamble to use
% it. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\long\def\realfig#1#2#3#4{
\begin{figure}[htbp]
%%%\centerline{\psfig{figure=#3,height=#2}}
\centerline{\psfig{figure=#2,width=#4}}
\caption[#1]{#3}
\oplabel{#1}
\end{figure}}

%&&&&&&&&&&&&       List of figures              &&&&&&&&&
%
%&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&

\newcommand{\comm}[1]{}
\newcommand{\comment}[1]{}
%\renewcommand{\marginpar}[1]{}




